Defensive Tensorization

We propose defensive tensorization, an adversarial defence technique that leverages a latent high-order factorization of the network. The layers of a network are first expressed as factorized tensor layers. Tensor dropout is then applied in the latent subspace, therefore resulting in dense reconstructed weights, without the sparsity or perturbations typically induced by the randomization.Our approach can be readily integrated with any arbitrary neural architecture and combined with techniques like adversarial training. We empirically demonstrate the effectiveness of our approach on standard image classification benchmarks. We validate the versatility of our approach across domains and low-precision architectures by considering an audio classification task and binary networks. In all cases, we demonstrate improved performance compared to prior works.

==> algo.tex <==
\algtext*{EndIf}
\algtext*{EndFor}
\begin{algorithm}[h]
\caption{Defensive tensorization}
\begin{algorithmic}[1]
\State \textbf{Input} sample \(\mytensor{X}_0\).
\For{\textbf{each} layer \(l\)}
 \State \textbf{Sample} random vector $\myvector{\lambda}_F, \cdots, \myvector{\lambda}_W \sim \text{Bernouilli}\left(\theta\right) $
 \State \textbf{Create} sketch matrices \(\mymatrix{M}_F  = \mydiag(\myvector{\lambda}_{F}), \cdots, \mymatrix{M}_W  = \mydiag(\myvector{\lambda}_{W}) \)
 \State \textbf{Sketch} the latent Core $\mytensor{\tilde G}_l = \mytensor{G}_l \times_0  \mymatrix{M}_F \times \cdots \times_{3} \mymatrix{M}_W$
 \State \textbf{Reconstruct} \(\mytensor{W}_k\) using Equation~(\ref{eq:bernouilli-tucker-weight}) \Comment{Randomized \emph{dense} reconstruction}
 \State \(\mytensor{X}_{l+1} \gets \Phi_l(\mytensor{W}_l \myconv \mytensor{X}_l)\) \Comment{Convolve $\mytensor{X}_l$ with the randomized reconstruction and apply $\Phi_l$}
\EndFor
\State \Return $\mytensor{X}_{L}$
\end{algorithmic}
\label{algorithm}
\end{algorithm}
